MatFormer: Nested Transformer for Elastic Inference

Foundation models are applied in a broad spectrum of settings with different inference constraints, from massive multi-accelerator clusters to resource-constrained standalone mobile devices. However, the substantial costs associated with training these models often limit the number of unique model sizes that can be offered. Consequently, practitioners are compelled to select a model that may not be optimally aligned with their specific latency and cost requirements. We present MatFormer, a novel Transformer architecture designed to provide elastic inference across diverse deployment constraints. MatFormer achieves this by incorporating a nested Feed Forward Network (FFN) block structure within a standard Transformer model. During training, we optimize the parameters of multiple nested FFN blocks with varying sizes, enabling the extraction of hundreds of accurate smaller models without incurring additional computational costs. We empirically validate the efficacy of MatFormer across different model classes (decoders and encoders) and modalities (language and vision), demonstrating its potential for real-world deployment. We show that a 850M decoder-only MatFormer language model (MatLM) allows us to extract multiple smaller models spanning from 582M to 850M parameters, each exhibiting better validation loss and one-shot downstream evaluations than independently trained counterparts. Furthermore, we observe that smaller encoders extracted from a universal MatFormer-based ViT (MatViT) encoder preserve the metric-space structure for adaptive large-scale retrieval. Finally, we showcase that speculative decoding with the accurate and consistent submodels extracted from MatFormer can lead to significant reduction in inference latency. Project website: https://devvrit.github.io/matformer/

==> sections/TabsNFigs/LM_MnMBaselineapp.tex <==
\begin{figure*}[t!]
\centering
% \vspace{-4mm}
% \begin{subfigure}[]{.7\textwidth}
  \centering
  \includegraphics[width=0.5\linewidth]{sections/TabsNFigs/images/850M_MnM_LossBaseline.pdf}
  % \label{fig:2B-mnm-loss-app}
% \end{subfigure}%
\caption{Validation loss for the 850M baseline models and their Mix'n'Match counterparts. Unlike MatLM, these extracted subnetworks perform poorly.}
\label{fig:lm_mnm-baseline-app}
\vspace{-2mm}
\end{figure*}


% \TS{MnM consistency}


==> sections/TabsNFigs/LM_MnMapp.tex <==
\begin{figure*}[t!]
\centering
\vspace{-2mm}
\begin{subfigure}[]{.33\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/2B_MnM_Lossapp.pdf}
  \caption{Validation loss}
  \label{fig:2B-mnm-loss-app}
\end{subfigure}%
\begin{subfigure}[]{.33\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/2B_MnM_Rankapp.pdf}
  \caption{1-shot RANK Evals}
  \label{fig:2B-mnm-rank-app}
\end{subfigure}
\begin{subfigure}[]{.33\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/2B_MnM_GENapp.pdf}
  \caption{1-shot GEN Evals}
  \label{fig:2B-mnm-gen-app}
\end{subfigure}
\caption{Validation loss \& one-shot downstream evaluation scores for the 2.6B MatLM \& baseline models. Mix'n'Match helps generate accurate models from MatLM that lie on the performance-vs-compute curve spanned by the explicitly optimized submodels.}
\label{fig:lm_mnm-app}
\vspace{-4mm}
\end{figure*}


% \TS{MnM consistency}


==> sections/TabsNFigs/SpeculativeDecoding.tex <==
% \begin{table}[h!]
% \centering
% \caption{Numbers for SPEED with 2.6B model}

% \begin{tabular}{ccc}
% \toprule
% Model for SPEED & XYZ dataset & ABC dataset \\\midrule
% 2.6B + 1B & B & C\\
% 2.6B + 1B (MatFormer) & &\\
% \bottomrule

% \end{tabular}
% \label{tab:spec_decode}
% \end{table}

% \begin{figure}
% \centering
% % \begin{subfigure}[]{.45\textwidth}
%   \centering
%   \includegraphics[width=0.5\linewidth]{sections/TabsNFigs/images/2B-Consistency.pdf}
%   \caption{Consistency for 2.6B}
%   \label{fig:consistency}
% % \end{subfigure}%
% \end{figure}%

% \begin{document}
  \begin{minipage}{\textwidth}
  \begin{minipage}[b]{0.49\textwidth}
    \centering
    \label{fig:consistency}
    \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/2B-Consistency.pdf}
    % \caption{Consistency for 2.6B}
    \captionof{figure}{Consistency of MatLM submodels' (L, M, S) predictions with the XL-model predictions compared against the consistency of comparable baselines with a baseline model as larger as the XL-model. The MatLM submodels are significantly more consistent with predictions of the XL-model compared to baselines, with the gap in consistency increasing for larger models.}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccc}
\toprule
Model for SPEED & XYZ dataset & ABC dataset \\\midrule
2.6B + 1B & B & C\\
2.6B + 1B (MatFormer) & &\\
\bottomrule
\label{tab:spec}
\end{tabular}}
      \captionof{table}{A table beside a figure}
    \end{minipage}
  \end{minipage}
% \end{document}

==> sections/TabsNFigs/evals_1.3B.tex <==
\begin{table}[]
\centering
\caption{\small Downstream Eval numbers and development set log perplexity loss on 1.3B model size granularities.}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{@{}l|llllllll@{}}
\toprule
Downstream Task         & Baseline-S & MatLM-S & Baseline-M & MatLM-M & Baseline-L & MatLM-L & Baseline-XL & MatLM-XL \\ \midrule
TriviaQA (EM) & 11.92 & 12 & 14.68 & 13.09 & 16.48 & 14.91 & 20.14 & 17.62 \\
NaturalQuestions (EM) & 1.88 & 2.19 & 2.24 & 2.47 & 3.07 & 2.99 & 4.79 & 4.13 \\
\midrule
WebQuestions (EM) & 3.84 & 5.02 & 4.72 & 5.36 & 5.07 & 5.76 & 6.05 & 6.15 \\
LAMBADA & 7.3 & 9.94 & 13.55 & 12.34 & 17.97 & 13.51 & 22.65 & 19.21 \\
HellaSwag & 40.53 & 40.35 & 42.86 & 42.5 & 46 & 44.48 & 49.78 & 47.69 \\
StoryCloze & 67.29 & 68.2 & 69.75 & 69.91 & 72.37 & 71.14 & 73.81 & 72.8 \\
\midrule
WSC & 64.56 & 65.96 & 64.91 & 69.12 & 67.72 & 69.82 & 72.63 & 69.82 \\
WinoGrande & 55.8 & 53.99 & 56.67 & 55.25 & 56.12 & 57.7 & 58.25 & 58.41 \\
Winograd & 71.06 & 68.5 & 67.77 & 70.7 & 73.99 & 70.33 & 72.53 & 72.89 \\
\midrule
SQuAD v2 (EM) & 29.63 & 35.47 & 28.85 & 34.64 & 36.55 & 34.47 & 39.48 & 36.39 \\
RACE-H & 32.19 & 33.19 & 33.08 & 34.39 & 34.48 & 35.11 & 36.59 & 35.25 \\
RACE-M & 43.8 & 44.22 & 44.22 & 45.96 & 47.7 & 45.75 & 50.07 & 46.59 \\
\midrule
PIQA & 66.49 & 64.36 & 66.05 & 66.38 & 67.52 & 66.97 & 69.1 & 67.68 \\
ARC-C & 27.99 & 25.77 & 27.65 & 27.22 & 29.01 & 28.75 & 30.55 & 31.48 \\
ARC-E & 56.44 & 54.08 & 58.54 & 57.03 & 59.85 & 58.84 & 63.26 & 61.83 \\
OpenBookQA & 41.4 & 42.2 & 41 & 42 & 43.4 & 42.8 & 44.8 & 45.4 \\
\midrule
BoolQ & 52.57 & 49.85 & 54.86 & 52.42 & 53.76 & 56.06 & 55.35 & 53.52 \\
COPA & 70 & 75 & 69 & 77 & 74 & 74 & 77 & 75 \\
RTE & 52.35 & 53.07 & 53.07 & 52.35 & 54.15 & 53.43 & 52.35 & 49.82 \\
WiC & 47.34 & 47.34 & 47.18 & 47.34 & 47.34 & 47.34 & 48.43 & 47.02 \\
MultiRC (F1) & 42.98 & 46.69 & 43.82 & 49.09 & 45.29 & 48.2 & 40.99 & 46.42 \\
ReCoRD & 67.32 & 67 & 69.02 & 68.61 & 71.13 & 70.26 & 73.4 & 71.49 \\
CB & 42.86 & 44.64 & 46.43 & 42.86 & 48.21 & 44.64 & 42.86 & 37.5 \\
\midrule
ANLI-R1 & 32.5 & 33.5 & 31.9 & 33.8 & 33 & 33.3 & 32.4 & 32.1 \\
ANLI-R2 & 30.3 & 34.7 & 30.5 & 34.6 & 30.6 & 33.1 & 31.5 & 33.5 \\
ANLI-R3 & 30.5 & 33.17 & 31.5 & 33.67 & 31.33 & 33.5 & 32.58 & 33.67 \\
\midrule
Average & 41.96 & 42.71 & 42.84 & 43.85 & 44.85 & 44.51 & 46.21 & 45.13 \\
\midrule
Avg over GEN Taks & 10.91 & 12.92 & 12.81 & 13.58 & 15.83 & 14.33 & 18.62 & 16.7 \\
\midrule
Avg over RANK Tasks & 49.35 & 49.8 & 49.99 & 51.06 & 51.76 & 51.69 & 52.77 & 51.9 \\
\midrule
Dev set log pplx & 2.90 & 2.923 & 2.856 & 2.867 & 2.79 & 2.81 & 2.718 & 2.76\\
\bottomrule
\end{tabular}}

\label{table:1.3bmevals}
\end{table}

==> sections/TabsNFigs/evals_2.6B.tex <==
\begin{table}[]
\centering
\caption{\small Downstream Eval numbers and development set log perplexity loss on 2.6B model size granularities.}
\vspace{-0.5em}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{@{}lllllllll@{}}
\toprule
Downstream Task         & Baseline-S & MatLM-S & Baseline-M & MatLM-M & Baseline-L & MatLM-L & Baseline-XL & MatLM-XL \\ \midrule
TriviaQA (EM) & 18.58 & 18.64 & 19.83 & 21.41 & 25.17 & 24.9 & 28.84 & 28.01 \\
NaturalQuestions (EM) & 3.05 & 3.13 & 3.19 & 3.66 & 4.76 & 4.24 & 6.73 & 5.01 \\
\midrule
WebQuestions (EM) & 5.61 & 6.74 & 4.43 & 6.3 & 6.1 & 6.74 & 8.27 & 7.78 \\
LAMBADA & 18.46 & 13.74 & 29.92 & 19.89 & 27.34 & 24.84 & 27.94 & 29.98 \\
HellaSwag & 46.41 & 46.01 & 49.04 & 48.94 & 52.87 & 52.2 & 57.14 & 55.33 \\
StoryCloze & 72.26 & 72.1 & 73.54 & 73.22 & 75.09 & 75.04 & 77.02 & 75.79 \\
\midrule
WSC & 71.23 & 69.82 & 70.88 & 71.58 & 75.09 & 74.39 & 80 & 77.54 \\
WinoGrande & 56.83 & 57.85 & 57.62 & 56.91 & 60.93 & 59.19 & 62.19 & 59.59 \\
Winograd & 76.56 & 71.43 & 72.89 & 74.36 & 76.56 & 74.73 & 81.68 & 78.75 \\
\midrule
SQuAD v2 (EM) & 34.89 & 37.97 & 34.33 & 40.07 & 34.89 & 42.24 & 43.47 & 42.59 \\
RACE-H & 33.62 & 34.76 & 35.59 & 35.85 & 36.91 & 36.82 & 38.91 & 37.28 \\
RACE-M & 47.63 & 47.49 & 49.44 & 49.51 & 50.77 & 50.07 & 53.34 & 51.67 \\
\midrule
PIQA & 67.74 & 67.79 & 68.39 & 68.28 & 69.21 & 69.59 & 71.49 & 71.11 \\
ARC-C & 29.95 & 30.29 & 31.83 & 31.91 & 32.51 & 34.22 & 35.67 & 35.41 \\
ARC-E & 60.82 & 59.97 & 61.2 & 62.42 & 63.51 & 64.56 & 67.76 & 64.86 \\
OpenBookQA & 45.6 & 43.8 & 45.4 & 44.8 & 49 & 46.4 & 49 & 49.4 \\
\midrule
BoolQ & 53.58 & 52.87 & 53.15 & 53.52 & 59.36 & 54.89 & 60.8 & 57.22 \\
COPA & 74 & 74 & 77 & 76 & 75 & 78 & 82 & 81 \\
RTE & 49.1 & 53.07 & 49.82 & 54.15 & 48.01 & 54.51 & 48.01 & 52.35 \\
WiC & 47.34 & 47.34 & 47.18 & 47.34 & 47.34 & 47.18 & 47.02 & 47.49 \\
MultiRC (F1) & 43.4 & 52.28 & 43.65 & 51.64 & 46.99 & 53.7 & 39.24 & 53.77 \\
ReCoRD & 71.34 & 71.9 & 72.79 & 72.97 & 74.86 & 74.57 & 76.71 & 75.32 \\
CB & 28.57 & 44.64 & 46.43 & 46.43 & 41.07 & 50 & 50 & 44.64 \\
\midrule
ANLI-R1 & 32.4 & 32.3 & 30.4 & 32.3 & 32.5 & 32.1 & 31.2 & 31.5 \\
ANLI-R2 & 30.4 & 30.1 & 30.6 & 31 & 30.1 & 30.2 & 31.7 & 30.8 \\
ANLI-R3 & 30.75 & 30.83 & 31.25 & 31 & 33.5 & 30.92 & 32 & 31.92 \\
\midrule
Average & 44.23 & 45.03 & 45.76 & 46.36 & 47.29 & 47.93 & 49.54 & 49.08 \\
\midrule
Avg over GEN Taks & 16.12 & 16.04 & 18.34 & 18.26 & 19.66 & 20.59 & 23.05 & 22.68 \\
\midrule
Avg over RANK Tasks & 50.93 & 51.94 & 52.29 & 53.05 & 53.86 & 54.44 & 55.85 & 55.37 \\
\midrule
Dev set log pplx & 2.77 & 2.787 & 2.722 & 2.732 & 2.66 & 2.68 & 2.592 & 2.63 \\
\bottomrule
\end{tabular}}
\label{table:2.6bevals}
\end{table}

==> sections/TabsNFigs/evals_2.6B_MnM.tex <==
\begin{table}[]
\centering
\caption{Downstream eval numbers and development set log perplexity on 2.6B MatLM Mix`n'Match granularities. For original granularities, please refer to \Cref{table:2.6bevals}. First row represents the non-embedding parameters of the model.}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{@{}l|lllllll@{}}
\toprule
Downstream Task         & 830M & 1B & 1.11B & 1.32B & 1.43B & 1.55B & 1.65B \\ \midrule
TriviaQA (EM) & 18.89 & 22.43 & 23.8 & 25.77 & 26.26 & 26.15 & 26.6 \\
NaturalQuestions (EM) & 3.49 & 3.77 & 4.02 & 4.07 & 4.46 & 4.65 & 5.12 \\
WebQuestions (EM) & 5.95 & 6.1 & 6.64 & 6.69 & 6.94 & 6.69 & 6.69 \\
LAMBADA & 16.34 & 20.16 & 23.07 & 24.8 & 24.32 & 25.87 & 29.13 \\
HellaSwag & 47.98 & 50.46 & 51.29 & 52.78 & 53.75 & 54.16 & 54.56 \\
StoryCloze & 73.01 & 73.33 & 74.83 & 75.2 & 75.68 & 75.41 & 75.63 \\
WSC & 70.88 & 70.53 & 74.04 & 72.98 & 74.74 & 73.33 & 77.19 \\
WinoGrande & 57.85 & 58.88 & 60.93 & 58.88 & 59.67 & 60.06 & 59.91 \\
Winograd & 73.26 & 73.26 & 76.19 & 74.36 & 76.56 & 77.66 & 78.02 \\
SQuAD v2 (EM) & 36.49 & 39.72 & 38.05 & 41.33 & 41.08 & 40.26 & 41.36 \\
RACE-H & 34.71 & 35.93 & 35.48 & 36.74 & 36.62 & 36.22 & 36.96 \\
RACE-M & 46.59 & 48.89 & 49.44 & 50.28 & 50.42 & 51.32 & 50.91 \\
PIQA & 68.5 & 69.04 & 69.53 & 70.4 & 70.46 & 70.51 & 70.29 \\
ARC-C & 31.06 & 33.11 & 33.19 & 34.81 & 35.75 & 35.84 & 34.56 \\
ARC-E & 62.29 & 62.58 & 62.63 & 64.86 & 65.99 & 65.49 & 64.69 \\
OpenBookQA & 44.6 & 46.2 & 46.8 & 47 & 47.4 & 47.4 & 47.6 \\
BoolQ & 54.86 & 55.08 & 54.46 & 55.78 & 58.38 & 57.19 & 56.88 \\
COPA & 76 & 76 & 75 & 80 & 77 & 80 & 80 \\
RTE & 53.43 & 53.79 & 53.79 & 52.71 & 53.79 & 54.51 & 53.79 \\
WiC & 47.34 & 47.34 & 47.18 & 47.34 & 47.18 & 47.34 & 48.12 \\
MultiRC (F1) & 53.34 & 53.85 & 52.97 & 54.23 & 57.57 & 55.09 & 54.91 \\
ReCoRD & 72.21 & 73.25 & 73.98 & 74.43 & 74.72 & 75.05 & 75.37 \\
CB & 48.21 & 46.43 & 48.21 & 50 & 50 & 44.64 & 55.36 \\
ANLI-R1 & 32.4 & 32.1 & 32 & 32.4 & 32.3 & 31.4 & 32.4 \\
ANLI-R2 & 30.5 & 30.6 & 30.6 & 30.6 & 30.7 & 30.4 & 31.4 \\
ANLI-R3 & 31.17 & 31.17 & 31.17 & 31.5 & 31 & 31.5 & 31.33 \\
Average & 45.82 & 46.69 & 47.28 & 48.07 & 48.57 & 48.39 & 49.18 \\
Avg over GEN Taks & 16.23 & 18.44 & 19.12 & 20.53 & 20.61 & 20.72 & 21.78 \\
Avg over RANK Tasks & 52.87 & 53.42 & 53.99 & 54.63 & 55.22 & 54.98 & 55.71 \\
\midrule
Dev set log pplx & 2.774 & 2.729 & 2.706 & 2.68 & 2.675 & 2.663 & 2.65\\
\bottomrule
\end{tabular}}
\label{table:2.6bmnm}
\end{table}

==> sections/TabsNFigs/ofa_plot.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{sections/TabsNFigs/images/850_OFA_Lossapp.pdf}
\caption{We compare an 850M OFA \citep{cai2019once} model with an 850M parameter MatFormer model. We find that whether we use Mix'n'Match or NAS, OFA results in a weaker final model.}
\label{fig:ofa}
\end{figure}

==> sections/TabsNFigs/optmethod.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h!]
\centering
\caption{We compared the validation loss of models from Joint Optimization to training MatLMs with independent MLP modules for each granularity (Independent modules) and sampling a single granularity to optimize for at each step (Subsampling) for 850M parameter models.}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 Model & {Training Strategy} & {XL} & {L} & {M} & {S} \\ \midrule
Baseline & - & {2.840} & {2.910} & {2.9710} & {3.017} \\\midrule
\multirow{3}{*}{MatFormer} & Joint Optimization & {2.874} & {2.928} & {2.980} & {3.030} \\
 & Independent MLP modules & {2.894} & {2.942} & {2.985} & {3.030} \\
 & Subsampling & 2.929 & 2.946 & 2.999 &	3.049   \\
 % \hdashline
 % \multirow{2}{*}{MatFormer - More Data} & Joint Optimization -- different batches & 2.852 & 2.893 & 2.943 &  2.977 \\ 
 % & Subsampling -- $4\times$ tokens & 2.848 & 2.886 & 2.934  &  2.97 \\ 
 \bottomrule
\end{tabular}%
}
\label{tab:opt}
\end{table}

==> sections/TabsNFigs/scaling_laws_64k.tex <==
\begin{figure*}
\centering
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.85\linewidth]{sections/TabsNFigs/images/XL-Scaling64k-Loss.pdf}
  \caption{XL-model Loss}
  \label{fig:XL-scaling64k}
\end{subfigure}%
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.85\linewidth]{sections/TabsNFigs/images/L-Scaling64k-Loss.pdf}
  \caption{L-model Loss}
  \label{fig:L-scaling64k}
\end{subfigure}
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/M-Scaling64k-Loss.pdf}
  \caption{M-model Loss}
  \label{fig:M-scaling64k}
\end{subfigure}
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/S-Scaling64k-Loss.pdf}
  \caption{S-model Loss}
  \label{fig:all-scaling64k}
\end{subfigure}

\begin{subfigure}[]{.45\textwidth}  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/all-Scaling64k-Loss.pdf}
  \caption{Loss for all granularities - XL, L, M, S}
  \label{fig:S-scaling64k}

  
\end{subfigure}
\caption{We train various decoder-only MatLM models at a range of sizes from 29M to 267M parameters with an embedding size of 64k and observe the scaling trends for each model granularity on validation loss. We observe that the gap between MatLM and the baseline appears to be constant at each granularity, similar to what is observed in Figure \ref{fig:scaling_laws}.}
\label{fig:scaling_laws64k}
\end{figure*}

==> sections/TabsNFigs/scaling_laws_dec.tex <==
% We perform a study of scaling laws with respect to model sizes inspired by recent work on the scaling laws of neural language models \cite{kaplan2020scaling,brown2020language}. Similar to their findings, our results show that model scaling improves our quality and that advantages of MatFormer doesn't degrade with scale. We plot the $4$ granularities of MatFormer and Baseline in \Cref{fig:scaling_laws} where we observe that both the Baseline and MatFormer scale similarly, with difference in log perplexity $<=0.03$ for any granularity and at any given scale. This difference in perplexity is within the error margin and doesn't affect downstream evals as we show in \Cref{fig:2B-mnm-gen,fig:2B-mnm-rank} for 2.6B model. Similar plots for other granularities are provided in the appendix.

% % Moreover, though we plot the granularities we explicitly trained for, we show in \Cref{fig:2B-mnm-loss} that using Mix`n'Match, we get many other models on the optimal loss-vs-size curve (within error margin). Moreover, downstream eval tasks on these Mix`n'Match granularities scale as well and lie on the optimal performance-vs-scale curve, as can be seen in \Cref{fig:2B-mnm-gen,fig:2B-mnm-rank}.


\begin{figure*}
\centering
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.85\linewidth]{sections/TabsNFigs/images/XL-Scalingdec-Loss.pdf}
  \caption{S-model Loss}
  \label{fig:XL-scalingdec}
\end{subfigure}%
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.85\linewidth]{sections/TabsNFigs/images/L-Scalingdec-Loss.pdf}
  \caption{S-model Loss}
  \label{fig:L-scalingdec}
\end{subfigure}
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/M-Scalingdec-Loss.pdf}
  \caption{S-model Loss}
  \label{fig:M-scalingdec}
\end{subfigure}
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/S-Scalingdec-Loss.pdf}
  \caption{Loss for all granularities - XL, L, M, S}
  \label{fig:all-scalingdec}
\end{subfigure}

\begin{subfigure}[]{.45\textwidth}  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/all-Scalingdec-Loss.pdf}
  \caption{All}
  \label{fig:S-scalingdec}

  
\end{subfigure}
\caption{We train various decoder-only MatLM models at a range of sizes from 78M to 2.6B parameters with a reweighing ratio of $2:1.5:1.25:1$ and observe the scaling trends for each model granularity on validation loss. We observe that the gap between MatLM and the baseline appears to be constant at each granularity, similar to what is observed in Figure \ref{fig:scaling_laws}.}
\label{fig:scaling_lawsdec}
\end{figure*}

==> sections/TabsNFigs/scaling_laws_gen.tex <==

\begin{figure*}
\centering
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.85\linewidth]{sections/TabsNFigs/images/XL-850M-Scaling-GPT3-GEN.pdf}
  \caption{XL-model Average Score on GEN tasks}
  \label{fig:XL-scaling-gen}
\end{subfigure}%
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.85\linewidth]{sections/TabsNFigs/images/L-850M-Scaling-GPT3-GEN.pdf}
  \caption{L-model Average Score on GEN tasks}
  \label{fig:L-scaling-gen}
\end{subfigure}
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/M-850M-Scaling-GPT3-GEN.pdf}
  \caption{M-model Average Score on GEN tasks}
  \label{fig:M-scaling-gen}
\end{subfigure}
\begin{subfigure}[]{.45\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/S-850M-Scaling-GPT3-GEN.pdf}
  \caption{S-model Average Score on GEN tasks}
  \label{fig:S-scaling-gen}
\end{subfigure}

\begin{subfigure}[]{.45\textwidth}  \includegraphics[width=0.8\linewidth]{sections/TabsNFigs/images/all-850M-Scaling-GPT3-GEN.pdf}
  \caption{Average Score on GEN tasks for all granularities - XL, L, M, S.}
  \label{fig:all-scaling-gen}

  
\end{subfigure}
\caption{We train various decoder-only MatLM models at a range of sizes from 78M to 850M parameters and observe the scaling trends for each model granularity for the average score on GEN tasks 1-shot evaluation. We observe that the gap between MatLM and the baseline reduces with scale, outperforming the baselines for S, M, L granularities for the largest models.}
\label{fig:scaling_laws_gen}
\end{figure*}

==> sections/TabsNFigs/transformer_costs.tex <==
% Please add the following required packages to your document preamble:

\begin{table}[h!]
\centering
\caption{Per-layer components and costs of a Transformer model per-token generation. $n$ is the sequence length, $d$ is the model dimension, $s$ is the scaling ratio of model dimension $\to$ hidden dimension, $h$ is the number of heads. The only two hyper-parameters are $h$ and $s$. $s$ controls the model capacity and often is either 4 or 8. Maybe we don't need MQA here}
\begin{tabular}{cccc}
\toprule
Component & Params & Complexity & Real-world Costs \\ \midrule
MLP       &  $2\cdot s\cdot d^2$ & $\mathcal{O}(2\cdot s\cdot d^2)$         &                 \\
MHA       &  $4\cdot d^2$ & $\mathcal{O}(4\cdot d^2 + n\cdot d)$         &                 \\\bottomrule
% MQA       &  $2\cdot (d^2 + d^2/h)$ & $\mathcal{O}(2\cdot (d^2 + d^2/h) + n\cdot d)$         &                 \\ \bottomrule
\label{tab:costs}
\end{tabular}
\end{table}

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:disc}
\TA{Improve in the later pass}

% \paragraph{Effect of vocabulary size on MatLM scaling laws.} Figure~\ref{fig:scaling_laws64k} in the appendix shows that vocabulary size does not have an effect on the scaling of MatLM which remains similar to a dense Transformer baseline even for the more ubiquitous 64K vocabulary size instead of our default 256K. 

% \paragraph{Effect of relative weighing of granularities in MatLM.} 
% Table~\ref{}. MatLM always relied on the hyperparameters from standard coutnerparts and were never searched for. However, an easy proxy is to reweight the granualrities as ablated in MRL. This helps find a way to further close the remaining minute gap. Further investigation based on muP should happen for both initialization and rewighting to have significant scaling improvements. 

% \paragraph{Effect of different training strategies.} While MatFormer relies on the joint optimization of prechosen granularities, the literature often preferred training of granularities through sampling one at a time~\citep{yu2018slimmable}. Table~\ref{} shows the empirical difference between joint training and training by sampling. Joint Training si significantly better.

% At the same time, one can also envision MatFormer as an MoE model where each expert is of varying size while being weight-tied. We investigate the effect of training a MatFormer with weight-separated experts of the same granularities. Table~\ref{} shows that the traditional MoE formulation with independent heads when optimized jointly performs consistently worse than a MatFormer model while having significantly more parameters.

Discussion:
\begin{itemize}
    \item Consistency as a desired property
    \item Position MatFormers within conditional compute
    \item Weight tying as a desired property
\end{itemize}

Future work:
\begin{itemize}
    \item further exploring weight tying within conditional compute
    \item better ways to select granularity to use 
    \item notions of training cost for future 
\end{itemize}

% \paragraph{Synergy between MatFormer and conditional compute.} All the previous experiments leveraging conditional compute with MatFormer showcase its effectiveness in static settings. However, MatFormer can be modified easily to enable dynamic compute like token-based routing or model selection from the universal XL model.  Similarly, a highly behavior-consistent pair of small and large MatFormer models can have a profound impact on minimizing communication costs and prediction drift between on-device and cloud deployments along with a plethora of speculative execution formulations. Finally, as argued earlier, MatFormer can be interpreted as a MoE model with weight-tied experts, which helps improving deployment aspects of MoEs with shared memory and compute among many other things.

\paragraph{Efficient implementations for MatFormers.} Training throughput of MatFormers can be improved significantly by using local gradient accumulation to reduce communication, and fused MatFormer kernels to fully utilize the hardware for smaller slices of the MatFormer. We discuss these algorithms in Appendix~\ref{app:efficiency}.

\paragraph{MatFormer scaling versus transformers.} MatFormers follow similar scaling behavior as regular transformers for the same hyperparameters, but initial experiments suggest that the right hyperparameters can improve MatFormer scaling. Furthermore, when combining training and deployment scaling laws with speculative decoding, we find that MatFormers use less overall FLOPS for the same performance when the number of inference tokens is approximately twice the number of training tokens. Details can be found in Appendix~\ref{app:scaling_laws}.


% MoE studd and other drifting and dynamic stuff

% \paragraph{Scaling laws of MatFormers vs Transformers.} Scaling laws are essential tools to estimate optimality under diverse viewpoints such as overall training cost in FLOPS, training data and parameter efficiency, and inference mean FLOPS utilization vs latency for deployments. The scaling relationship of MatFormers versus transformers is both simple and complex. Simple, because MatFormers the scaling curves for pretraining are only slightly offset from transformers -- thus matformers only require a fixed relative amount of additional compute and the same hyperparameters that work for transformers are effective for matformers. The complex relationship comes that the MatFormer allows the training of multiple models with a single training run which is a qualitative different from transformers and difficult to factor into scaling equations. Essentially, in terms of efficiency, MatFormers have a clear advantage in any case where a model is trained and a smaller model is also desirable. One straightforward of these cases is speculative decoding which allows a tradeoff between FLOPs per sample and latency during inference -- more FLOPs are used per token, but the overall latency is decreased. Since MatFormers provide better agreement for the models in speculative decoding, Matformers provide better cost efficiency. Depending on the improvement in speculative decoding we can use scaling behavior of matformers vs transformers to estimate when training and deploying a matformer is cheaper than training a single transformer and using an already trained transformer.

% \paragraph{Improving MatFormer Training Efficiency.} While MatFormer training uses asymptotically 2x FLOPs compared to a regular transformer optimizations are necessary to also realize a 2x runtime training performance. {\bf Delayed gradient synchronization via local accumulation: } Since multiple forward and backward passes are made for each mini-batch in common implementations of data parallelism this induces a gradient synchronization across all device for each backward pass with additional gradient accumulation. As such, a minimum of 2x the parameters worth of gradients are exchanged for the MLP layers, thus increasing the communication overhead. Additionally, for some frameworks, such as PyTorch, gradients of the full weight matrix size need to be exchanged, leading to 4x more communication for our default experimental setup. A more efficient way to communicate gradients is to keep a local gradient accumulation buffer, which is used to accumulate all gradient from all subnetworks into the main, full-sized weight gradient. After all forward-backward passes have been completed, synchronization of gradients -- with additional overall of computation and communication -- can ensue. This saves 2x communication overhead, reducing communication overhead to the same cost as a regular transformer. {\bf Fused matformer kernels:} Depending on the accelerator (GPU/TPU), the smallest MatFormer forward and backward pass can be inefficient in that the matrices are too small to fully utilize the accelerator. To improve utilization at the cost of additional memory for activations it is possible to run the following computational fusion strategy for matformer computation: (a) duplicate mini-batch 4x, (b) do the forward/backward pass for each layer for all matformer stages at the same time, (c) in doing so, load the tile for the weight matrix once, and reuse it for all relevant matformer stages. This strategy is similar to tiling strategies in FlashAttention~\citep{dao2022flashattention} or convolution~\citep{krizhevsky2009convolutional} which increase the arithmetic intensity for small weights by reusing of matrix multiplication tiles written to SRAM. 

%\paragraph{Return of investments of MatFormer training and deployment vs transformers.} Given the case that we have the choice of training and deploying a matformer versus a transformer with speculative decoding, we can ask, what is the crossing point where matformer training and deployment is cheaper than the training and deployment of a transformer. Since training a single matformer is always cheaper than training a transformer main model and a transformer draft model, the most important case to compare against is the following case: (A) We train and deploy a matformer with specualative decoding; (B) We train a transformer and deploy a previously trained smaller transformer as a draft model for speculative decoding. To make this comparison fair, we need to control for the latency of both approaches. We additionally assume that mean FLOPs utilization is approximately equal in both cases. In our experiments, we have shown that matformers with MLP layers 1/8th the size of the full model always has better agreement than a transformer with full MLP layers trained from scratch. Since MLP layers usually  have $2\times 4h \times h$ parameters and attention layers $4\times h \times h$ parameters, where $h$ is the transformer model dimension, this means that the MLP layers contain 8:4 = 8/12 = 67\% of parameters. Thus a transformer draft model for speculative decoding with $P$ parameters is always higher latency compared to a matformer with $0.33P + \frac{0.66P}{8} = 0.4125P$ parameters. 

\begin{itemize}
    % \item Effect of vocab size
    % \item effect of reweiging
    % \item Effect of joint training vs sampling (which is common)
    % \item MatFormer vs MoE (Conditional Layer arguments)
    \item Arguments about scaling laws based on "wall clock cost" and the free Mix'n'Match models being ignore (normalized scaling laws?) and potential kernel fusing and better GPU utils. \textbf{TODO: Tim}
    % \item Other potential downstream uses -- variety of speculative decoding, consitent models across cloud and edge for minimal drift and anything else?  \textbf{TODO: Tim}
\end{itemize}

==> sections/introduction_v2.tex <==



Series of models - train only a few models 

33B (x FLOPs) and 65 B (y FLOPs). Training a new variant would take Z FLOPs. 
ALSO - inference schemes that use co=location are popular.

Whereas before - Z FLOPS, this can be obtained for no additional compute 
No compression or quality loss.

redo order of Matformer bullet points THEN intro

==> sections/repro_statement.tex <==
\section*{Reproducibility Statement}
The architecture description and the model training procedures are clearly outlined in Section~\ref{sec:method}. MatFormer can be induced with ease in any Transformer by introducing matryoshka structure~\citep{kusupati2022matryoshka} on the hidden representation of the FFN block. All the experiments on language modelling can be executed on any large text corpus while all the computer vision experiments are performed on the standard ImageNet~\citep{deng2009imagenet,russakovsky2015imagenet} benchmark using the Scenic library~\citep{dehghani2022scenic}. Lastly, we have described more implementation, training and evaluation details in Appendix~\ref{app:impl} and further training optimizations in Appendix~\ref{app:efficiency}.
